Mixed Attention Transformer for Leveraging Word-Level Knowledge to Neural Cross-Lingual Information Retrieval

Pretrained contextualized representations offer great success for many downstream tasks, including document ranking. The multilingual versions of such pretrained representations provide a possibility of jointly learning many languages with the same model. Although it is expected to gain big with such joint training, in the case of cross lingual information retrieval (CLIR), the models under a multilingual setting are not achieving the same level of performance as those under a monolingual setting. We hypothesize that the performance drop is due to the translation gap between query and documents. In the monolingual retrieval task, because of the same lexical inputs, it is easier for model to identify the query terms that occurred in documents. However, in the multilingual pretrained models that the words in different languages are projected into the same hyperspace, the model tends to translate query terms into related terms, i.e., terms that appear in a similar context, in addition to or sometimes rather than synonyms in the target language. This property is creating difficulties for the model to connect terms that cooccur in both query and document. To address this issue, we propose a novel Mixed Attention Transformer (MAT) that incorporates external word level knowledge, such as a dictionary or translation table. We design a sandwich like architecture to embed MAT into the recent transformer based deep neural models. By encoding the translation knowledge into an attention matrix, the model with MAT is able to focus on the mutually translated words in the input sequence. Experimental results demonstrate the effectiveness of the external knowledge and the significant improvement of MAT embedded neural reranking model on CLIR task.

==> sections/01-introduction.tex <==
\section{Introduction}  \label{sec:introduction}

Pre-trained Transformer-based  models such as BERT~\cite{devlin-etal-2019-bert} have shown promising performance gains in many downstream tasks including document retrieval~\cite{jiang-etal-2020-cross, qiao2019understanding,yates-etal-2021-pretrained,10.1145/3397271.3401325}. This success is mainly due to the unsupervised pre-training of context-aware architectures -- with an  enormous number of parameters -- over a large corpora. To achieve success in the learning-to-rank task such models are often fine-tuned with a relatively large collection of relevance judgments such as the MS MARCO  passage ranking dataset~\cite{nogueira2019passage}. It is not feasible to obtain data in the scale of MS MARCO for a variety of different domains and languages. Thus, some studies leverage different training data (e.g., weak-supervised data, cross-lingual Wikipedia-based data~\cite{sasaki2018cross,schamoni2014learning}) and techniques (e.g., domain adaptation, few-shot learning) in order to adapt the model for the target task and language, reporting improvements. 

We study the problem of Cross-Lingual Information Retrieval (CLIR) in which the desired information is written in a human language which is different than that of the user’s query. From the modeling perspective, with the CLIR setting some form of language translation is needed to map  the vocabulary of the query language to that of the documents’ language in addition to the ranking component. This form of translation medium ranges from simple dictionaries, translation tables, machine translation, and more recently cross-language distributional representations. Embedding the translation component along with the ranking makes the training of deep neural CLIR re-ranking models more challenging particularly when dealing with resource-lean non-English languages~\cite{10.1145/3341981.3344236,10.1145/3331184.3331324}. 

The multilingual versions of pre-trained Transformer-based language models such as mBERT \cite{devlin-etal-2019-bert} and XLM-R \cite{conneau2020unsupervised} makes it possible to jointly learn many languages within the same model. Although significant gain is expected from a unified language representation space, model fine-tuning in this multilingual setting is not achieving the same level of performance as the monolingual setting~\cite{litschko2018unsupervised}. 
For example, in a bilingual CLIR scenario, the vocabulary size is almost doubled, the exact match possibility between query and document is limited, and there is scarce publicly available training data (e.g., bilingual query log or click data). To this end, most of the existing CLIR systems are deployed along with a query translation component to reduce the problem into monolingual retrieval. However, it is important to note that having a translation component as a black-box limits the retrieval component due to translation errors. 
%  \rab{some brief overview of the recent existing works on the CLIR domain. }
% \rab{explain multilingual pre-trained models }
In the multilingual pre-trained models, even if the words in different languages are projected into the same hyperspace, the model tends to map query terms into target language's related terms – i.e., terms that appear in a similar context – in addition to or sometimes rather than synonyms. We hypothesize that this phenomena is creating difficulties for the model to connect terms that co-occur in both query and document. It has been shown that the translation gap is a key factor for the suboptimal performance of neural CLIR models and addressing that can significantly boost the retrieval performance~\cite{bonab2020training}. 

In contrast to the data-driven approach taken by~\citet{bonab2020training}, we inject word-level translation knowledge into a model at the time of fine-tuning it with relevance data.  More specifically, we leverage the external knowledge in the form of a translation table, which is a look-up table that provides translation probabilities for a pair of words in two different languages. We use the translation table to create an attention matrix and use it in parallel with the Transformer’s multi-head attention -- both in our training and inference phase -- to improve the model's cross-lingual understanding. We refer to our extended component as Mixed Attention Transformer (MAT) and create MART, a sandwich-like architecture to embed MAT into the multilingual BERT (mBERT) model. By encoding the translation knowledge into an attention matrix, we enable the overall architecture to focus on the mutually translated words in the input sequence. Our experiments explore the effectiveness of a variety of external knowledge sources and show the significant gain that we get from MART on CLIR task. MAT is a generalized architecture capable to capture any form of lexical mapping and it can be integrated with any transformer-based architecture. 


%We believe our modeling of the neural CLIR system dramatically reduces the need for cross-lingual ranking training data. 

The rest of this paper is organized as follows. In Section 2 we provide a review of related works. Section 3 presents our MAT architecture for injecting external translation knowledge directly into model. Section 4 and 5 provides our experimental design and results with a some discussions and further analyses. We conclude our study in Section 6. 







